Developer-Intent Driven Code Comment Generation

Existing automatic code comment generators mainly focus on producing a general description of functionality for a given code snippet without considering developer intentions. However, in real-world practice, comments are complicated, which often contain information reflecting various intentions of developers, e.g., functionality summarization, design rationale, implementation details, code properties, etc. To bridge the gap between automatic code comment generation and real-world comment practice, we define Developer-Intent Driven Code Comment Generation, which can generate intent-aware comments for the same source code with different intents. To tackle this challenging task, we propose DOME, an approach that utilizes Intent-guided Selective Attention to explicitly select intent-relevant information from the source code, and produces various comments reflecting different intents. Our approach is evaluated on two real-world Java datasets, and the experimental results show that our approach outperforms the state-of-the-art baselines. A human evaluation also confirms the significant potential of applying DOME in practical usage, enabling developers to comment code effectively according to their own needs.

==> TODO.tex <==
完成一稿：8.31中午


8.30
陈啸 卓浩
第五章 实验表V  1
定性分析例子-图表
RQ3 图
RQ3文字填空
paper website  1

8.30
方文：

第三章尾巴 1

第四章补充result 1

第五章 
实验表数据给陈啸  1
RQ1、RQ2结果分析* 1
RQ3 预填一个模板 1

第六章
定性分析*-文字
找两个例子 1
threat复用  1

第七章
相关工作-usage comment生成

结论
摘要* 1


更新图标的标题


8.31
定性分析-图-陈啸
RQ3-图
motivation更新-陈啸

定性分析-文字-方文*
RQ3文字-方文
结论-方文
Fix comment-方文

相关工作-usage comment生成-TBD



=======
question:
intents or intent or intention?
sub-layer

9.1
定性分析图-陈啸 1 
定性分析attention图-陈啸
HE图数据更新、压缩-陈啸
Motivation图更新（用case1)-陈啸 1

方文：
1-intro
2-3个表/图对应的问题（标注工具、RQ1、RQ3）
3-定性分析文字-方文 
Fix comment-方文 



压缩空间:  - 涵芝
Table V 调整 1
Fig 2 压扁 1

application study 都写成human evaluation

相关工作-usage comment生成-TBD



9.2
陈啸
调整空间
调整图表位置

检查所有数字

检查图表: 位置是否合适，标题是否合适，是否每个图表文字都引用？是否每个引用都正确？
Proof Reading
review 参考文献

方文
内容检查、逻辑检查
proof reading
intent-specific 都改成 intent-aware

涵芝
编辑参考文献

==> sec/0.abs-v2.tex <==
\begin{abstract}
%The goal of code comment generation is to generate a concise and fluent comment for a given code snippet. 

Most code summarization approaches pursue a general representation of code-comment relations and use the same treatment to generate different kinds of comments. However, comments are complicated in practice, e.g., 
developers may describe not only the functionality but also the design rationale and implementation details for one code snippet in a comment.


{To bridge the gap, we define On-Demand Code Comment Generation, which is a one-to-many mapping task, requiring model can generate intent-aware comments given the same source code and different intents of developers. To tackle this challenging task, we propose DOME, an approach that utilizes the Intent-guided Selective Attention to explicitly select intent-relevant information from the source code, and produces various comments reflecting different intents.} 
Our approach is evaluated on two real-world Java datasets, and the experimental results show that our approach outperforms the state-of-the-art baselines. 
A human evaluation also confirms the significant potential of applying {\tool} in practical usage, for enabling developers to comment code effectively according to their own needs.

% Inspired by this, in this work, we first propose a new task called On-Demand Comment Generation, which aims to create a comment that is coherent with the given developer's intent. Then, we develop an comment-intent classifier to support the automatic annotation of comment intents. Finally, we design a novel model, named {\tool}, which learns a one-to-many mapping and can generate various comments reflecting different intent.

\end{abstract}

==> sec/website.tex <==


% website: https://github.com/ICSE-DOME/DOME

% github account: ICSE_DOME
%        password: DOME_icse_20220830
%        username:ICSE-DOME
% mail address: ICSE23_DOME@outlook.com
%        password:DOME_icse_20220830

==> tab/RQ1.tex <==

\begin{table*}[hbtp!]
\centering
\caption{{Performances of {\tool} and baselines on each intent category}}
\label{table:RQ1}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{cc|cccc|cccc}
\hline
\multirow{2}{*}{Intent}   & \multirow{2}{*}{Methods} & \multicolumn{4}{c}{Funcom}                                   & \multicolumn{4}{c}{TLC}                                  \\
\cline{3-10}
                          &                          & BLEU           & ROUGE-L        & METEOR         & CIDEr     & BLEU           & ROUGE-L        & METEOR         & CIDEr \\
\hline
\multirow{4}{*}{What}     & Rencos                   & 26.19          & 31.10          & 14.61          & 0.00      & 23.28          & 36.89          & 16.02          & 0.00  \\
                          & EditSum                  & 27.58          & 31.06          & 14.24          &           & 21.34          & 33.73          & 13.42          &       \\
                          & AST-Trans                & 27.84          & 38.28          & 18.49          &           & 23.42          & 34.24          & 17.17          &       \\\hline
                          & DOME                     & \textbf{33.29} & \textbf{41.67} & \textbf{20.53} & \textbf{} & \textbf{25.39} & \textbf{39.56} & \textbf{18.22} &       \\
                          &DOME  \textit{w/o ISA} & 32.01 &38.74 & 18.65 & & 24.37& 37.93 & 16.51 & 
                          \\
                          \hline \hline
\multirow{4}{*}{Why}      & Rencos                   & 24.81          & 30.12          & 14.21          &           & 20.55          & 32.99          & 14.54          &       \\
                          & EditSum                  & 27.17          & 30.98          & 14.66          &           & 18.42          & 29.85          & 11.81          &       \\
                          & AST-Trans                & 25.96          & 35.74          & 17.77          &           & 19.31          & 29.37          & 14.94          &       \\
                          & DOME                     & \textbf{33.07} & \textbf{42.31} & \textbf{20.56} & \textbf{} & \textbf{21.97} & \textbf{35.31} & \textbf{15.77} &       \\
                          \hline
\multirow{4}{*}{Usage}    & Rencos                   & 25.54          & 27.74          & 13.34          &           & 14.62          & 22.61          & 10.21          &       \\
                          & EditSum                  & 25.25          & 27.25          & 12.79          &           & 14.00          & 21.51          & 9.07           &       \\
                          & AST-Trans                & 24.93          & 30.90          & 15.09          &           & 13.24          & 18.20          & 9.16           &       \\
                          & DOME                     & \textbf{31.63} & \textbf{39.31} & \textbf{19.34} & \textbf{} & \textbf{17.16} & \textbf{26.11} & \textbf{12.36} &       \\
                          \hline
\multirow{4}{*}{Done}     & Rencos                   & 19.84          & 29.28          & 12.53          &           & 18.58          & 33.73          & 13.12          &       \\
                          & EditSum                  & 22.22          & 29.73          & 12.62          &           & 16.84          & 31.18          & 11.12          &       \\
                          & AST-Trans                & 19.65          & 33.60          & 14.40          &           & 17.61          & 30.32          & 13.29          &       \\
                          & DOME                     & \textbf{26.98} & \textbf{39.52} & \textbf{17.65} & \textbf{} & \textbf{20.48} & \textbf{36.66} & \textbf{14.73} &       \\
                          \hline
\multirow{4}{*}{Property} & Rencos                   & 25.57          & 35.60          & 16.39          &           & 23.82          & 38.85          & 17.76          &       \\
                          & EditSum                  & 26.79          & 36.09          & 16.60          &           & 22.35          & 37.74          & 16.33          &       \\
                          & AST-Trans                & 28.29          & 43.54          & 20.73          &           & 23.54          & 36.56          & 18.47          &       \\
                          & DOME                     & \textbf{34.18} & \textbf{49.43} & \textbf{24.32} & \textbf{} & \textbf{26.01} & \textbf{45.73} & \textbf{21.29} &       \\
                          \hline
\multirow{4}{*}{Average}  & Rencos                   & 24.39          & 30.77          & 14.22          &           & 20.17          & 33.01          & 14.33          &       \\
                          & EditSum                  & 25.80          & 31.02          & 14.18          &           & 18.59          & 30.80          & 12.35          &       \\
                          & AST-Trans                & 25.33          & 36.41          & 17.30          &           & 19.42          & 29.74          & 14.61          &       \\
                          & DOME                     & \textbf{31.83} & \textbf{42.45} & \textbf{20.48} & \textbf{} & \textbf{22.20} & \textbf{36.67} & \textbf{16.47} &    
                          \\
                          \hline
\end{tabular}
}
\end{table*}

==> tab/RQ1andRQ2.tex <==

\begin{table*}[tp!]
\centering
\caption{{Performances of {\tool} and baselines on each intent category}}
\label{table:RQ1andRQ2}
%\setlength{\tabcolsep}{3pt}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{c|c|c|ccc|ccc}
\hline
\multirow{2}{*}{Intent}   & \multicolumn{2}{c|}{\multirow{2}{*}{Method}}  & \multicolumn{3}{c}{Funcom}                       & \multicolumn{3}{c}{TLC}                          \\\cline{4-9}
                          & \multicolumn{2}{c|}{}                         & BLEU           & ROUGE-L        & METEOR         & BLEU           & ROUGE-L        & METEOR         \\
                          \hline
\multirow{6}{*}{What}     & \multirow{3}{*}{Baseline}     & Rencos       & 26.19          & 31.10          & 14.61          & 23.28          & 36.89          & 16.02          \\
                          &                               & EditSum      & 27.58          & 31.06          & 14.24          & 21.34          & 33.73          & 13.42          \\
                          &                               & AST-Trans    & 27.84          & 38.28          & 18.49          & 23.42          & 34.24          & 17.17          \\\cline{2-9}
                          & \multirow{3}{*}{\makecell{Our \\Approach}} & DOME         & \textbf{33.29} & \textbf{41.67} & \textbf{20.53} & \textbf{25.39} & \textbf{39.56} & \textbf{18.22} \\
                          &                               & DOME \textit{w/o ISA} & 32.01          & 38.74          & 18.65          & 24.37          & 37.93          & 16.51          \\
                          &                               & DOME \textit{w/o ER}  & 31.33          & 38.12          & 18.57          & 23.82          & 37.24          & 16.37          \\
                          \hline
\multirow{6}{*}{Why}      & \multirow{3}{*}{Baseline}     & Rencos       & 24.81          & 30.12          & 14.21          & 20.55          & 32.99          & 14.54          \\
                          &                               & EditSum      & 27.17          & 30.98          & 14.66          & 18.42          & 29.85          & 11.81          \\
                          &                               & AST-Trans    & 25.96          & 35.74          & 17.77          & 19.31          & 29.37          & 14.94          \\\cline{2-9}
                          & \multirow{3}{*}{\makecell{Our \\Approach}} & DOME         & \textbf{33.07} & \textbf{42.31} & \textbf{20.56} & \textbf{21.97} & \textbf{35.31} & \textbf{15.77} \\
                          &                               & DOME \textit{w/o ISA} & 31.79          & 39.37          & 19.11          & 21.41          & 34.27          & 15.56          \\
                          &                               & DOME \textit{w/o ER}  & 31.13          & 38.78          & 18.99          & 19.60          & 32.16          & 12.71          \\
                          \hline
\multirow{6}{*}{How-to-use}    & \multirow{3}{*}{Baseline}     & Rencos       & 25.54          & 27.74          & 13.34          & 14.62          & 22.61          & 10.21          \\
                          &                               & EditSum      & 25.25          & 27.25          & 12.79          & 14.00          & 21.51          & 9.07           \\
                          &                               & AST-Trans    & 24.93          & 30.90          & 15.09          & 13.24          & 18.20          & 9.16           \\\cline{2-9}
                          & \multirow{3}{*}{\makecell{Our \\Approach}} & DOME         & \textbf{31.63} & \textbf{39.31} & \textbf{19.34} & \textbf{17.16} & \textbf{26.11} & \textbf{12.36} \\
                          &                               & DOME \textit{w/o ISA} & 30.57          & 37.24          & 17.54          & 16.74          & 25.59          & 11.25          \\
                          &                               & DOME \textit{w/o ER}  & 30.42          & 37.15          & 17.37          & 15.33          & 24.96          & 10.94          \\
                          \hline
\multirow{6}{*}{How-it-is-done}     & \multirow{3}{*}{Baseline}     & Rencos       & 19.84          & 29.28          & 12.53          & 18.58          & 33.73          & 13.12          \\
                          &                               & EditSum      & 22.22          & 29.73          & 12.62          & 16.84          & 31.18          & 11.12          \\
                          &                               & AST-Trans    & 19.65          & 33.60          & 14.40          & 17.61          & 30.32          & 13.29          \\\cline{2-9}
                          & \multirow{3}{*}{\makecell{Our \\Approach}} & DOME         & \textbf{26.98} & \textbf{39.52} & \textbf{17.65} & \textbf{20.48} & \textbf{36.66} & \textbf{14.73} \\
                          &                               & DOME \textit{w/o ISA} & 26.03          & 38.19          & 18.20          & 19.50          & 36.57          & 13.10          \\
                          &                               & DOME \textit{w/o ER}  & 25.78          & 37.73          & 18.10          & 19.14          & 35.72          & 13.01          \\
                          \hline
\multirow{6}{*}{Property} & \multirow{3}{*}{Baseline}     & Rencos       & 25.57          & 35.60          & 16.39          & 23.82          & 38.85          & 17.76          \\
                          &                               & EditSum      & 26.79          & 36.09          & 16.60          & 22.35          & 37.74          & 16.33          \\
                          &                               & AST-Trans    & 28.29          & 43.54          & 20.73          & 23.54          & 36.56          & 18.47          \\\cline{2-9}
                          & \multirow{3}{*}{\makecell{Our \\Approach}} & DOME         & \textbf{34.18} & \textbf{49.43} & \textbf{24.32} & \textbf{26.01} & \textbf{45.73} & \textbf{21.29} \\
                          &                               & DOME \textit{w/o ISA} & 32.21          & 46.92          & 22.70          & 25.35          & 43.68          & 19.47          \\
                          &                               & DOME \textit{w/o ER}  & 31.80          & 46.09          & 21.59          & 25.01          & 42.85          & 19.16          \\
                          \hline\hline
\multirow{6}{*}{\textit{Average}}  & \multirow{3}{*}{Baseline}     & Rencos       & 24.39          & 30.77          & 14.22          & 20.17          & 33.01          & 14.33          \\
                          &                               & EditSum      & 25.80          & 31.02          & 14.18          & 18.59          & 30.80          & 12.35          \\
                          &                               & AST-Trans    & 25.33          & 36.41          & 17.30          & 19.42          & 29.74          & 14.61          \\\cline{2-9}
                          & \multirow{3}{*}{\makecell{Our \\Approach}} & DOME         & \textbf{31.83} & \textbf{42.45} & \textbf{20.48} & \textbf{22.20} & \textbf{36.67} & \textbf{16.47} \\
                          &                               & DOME \textit{w/o ISA} & 30.52          & 40.09          & 19.24          & 21.47          & 35.61          & 15.18          \\
                          &                               & DOME \textit{w/o ER}  & 30.09          & 39.57          & 18.92          & 20.58          & 34.59          & 14.44 \\\hline        
\end{tabular}
}
\end{table*}

==> tab/RQ2.tex <==
\begin{table}[hbtp!]
\centering
\caption{{Ablation study on the ISA and Exemplar.}}
\label{table:RQ2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccc|ccc|}
\hline
\multirow{2}{*}{Intent}   & \multirow{2}{*}{Method}            & \multicolumn{3}{c|}{Funcom}                                        & \multicolumn{3}{c|}{TLC}                                           \\ \cline{3-8} 
                          &                              & \multicolumn{1}{c|}{BLEU}  & \multicolumn{1}{c|}{ROUGE-L} & METEOR & \multicolumn{1}{c|}{BLEU}  & \multicolumn{1}{c|}{ROUGE-L} & METEOR \\ \hline
\multirow{3}{*}{What}     & DOME w/o ISA & \multicolumn{1}{c|}{32.01} & \multicolumn{1}{c|}{38.74}   & 18.65  & \multicolumn{1}{c|}{24.37} & \multicolumn{1}{c|}{37.93}   & 16.51  \\ \cline{2-8} 
                          & DOME w/o Exemplar  & \multicolumn{1}{c|}{31.33} & \multicolumn{1}{c|}{38.12}   & 18.57  & \multicolumn{1}{c|}{23.82} & \multicolumn{1}{c|}{37.24}   & 16.37  \\ \cline{2-8} 
                          & DOME                         & \multicolumn{1}{c|}{33.29} & \multicolumn{1}{c|}{41.67}   & 20.53  & \multicolumn{1}{c|}{25.39} & \multicolumn{1}{c|}{39.56}   & 18.22  \\ \hline
\multirow{3}{*}{Why}      & DOME w/o ISA & \multicolumn{1}{c|}{31.79} & \multicolumn{1}{c|}{39.37}   & 19.11  & \multicolumn{1}{c|}{21.41} & \multicolumn{1}{c|}{34.27}   & 15.56  \\ \cline{2-8} 
                          & DOME w/o Exemplar  & \multicolumn{1}{c|}{31.13} & \multicolumn{1}{c|}{38.78}   & 18.99  & \multicolumn{1}{c|}{19.60} & \multicolumn{1}{c|}{32.16}   & 12.71  \\ \cline{2-8} 
                          & DOME                         & \multicolumn{1}{c|}{33.07} & \multicolumn{1}{c|}{42.31}   & 20.56  & \multicolumn{1}{c|}{21.97} & \multicolumn{1}{c|}{35.31}   & 15.77  \\ \hline
\multirow{3}{*}{Usage}    & DOME w/o ISA & \multicolumn{1}{c|}{30.57} & \multicolumn{1}{c|}{37.24}   & 17.54  & \multicolumn{1}{c|}{16.74} & \multicolumn{1}{c|}{25.59}   & 11.25  \\ \cline{2-8} 
                          & DOME w/o Exemplar  & \multicolumn{1}{c|}{30.42} & \multicolumn{1}{c|}{37.15}   & 17.37  & \multicolumn{1}{c|}{15.33} & \multicolumn{1}{c|}{24.96}   & 10.94  \\ \cline{2-8} 
                          & DOME                         & \multicolumn{1}{c|}{31.63} & \multicolumn{1}{c|}{39.31}   & 19.34  & \multicolumn{1}{c|}{17.16} & \multicolumn{1}{c|}{26.11}   & 12.36  \\ \hline
\multirow{3}{*}{Done}     & DOME w/o ISA & \multicolumn{1}{c|}{26.03} & \multicolumn{1}{c|}{38.19}   & 18.20  & \multicolumn{1}{c|}{19.50} & \multicolumn{1}{c|}{36.57}   & 13.10  \\ \cline{2-8} 
                          & DOME w/o Exemplar  & \multicolumn{1}{c|}{25.78} & \multicolumn{1}{c|}{37.73}   & 18.10  & \multicolumn{1}{c|}{19.14} & \multicolumn{1}{c|}{35.72}   & 13.01  \\ \cline{2-8} 
                          & DOME                         & \multicolumn{1}{c|}{26.98} & \multicolumn{1}{c|}{39.52}   & 17.65  & \multicolumn{1}{c|}{20.48} & \multicolumn{1}{c|}{36.66}   & 14.73  \\ \hline
\multirow{3}{*}{Proeprty} & DOME w/o ISA & \multicolumn{1}{c|}{32.21} & \multicolumn{1}{c|}{46.92}   & 22.70  & \multicolumn{1}{c|}{25.35} & \multicolumn{1}{c|}{43.68}   & 19.47  \\ \cline{2-8} 
                          & DOME w/o Exemplar  & \multicolumn{1}{c|}{31.80} & \multicolumn{1}{c|}{46.09}   & 21.59  & \multicolumn{1}{c|}{25.01} & \multicolumn{1}{c|}{42.85}   & 19.16  \\ \cline{2-8} 
                          & DOME                         & \multicolumn{1}{c|}{34.18} & \multicolumn{1}{c|}{49.43}   & 24.32  & \multicolumn{1}{c|}{26.01} & \multicolumn{1}{c|}{45.73}   & 21.29  \\ \hline
\multirow{3}{*}{Average}  & DOME w/o ISA & \multicolumn{1}{c|}{30.52} & \multicolumn{1}{c|}{40.09}   & 19.24  & \multicolumn{1}{c|}{21.47} & \multicolumn{1}{c|}{35.61}   & 15.18  \\ \cline{2-8} 
                          & DOME w/o Exemplar  & \multicolumn{1}{c|}{30.09} & \multicolumn{1}{c|}{39.57}   & 18.92  & \multicolumn{1}{c|}{20.58} & \multicolumn{1}{c|}{34.59}   & 14.44  \\ \cline{2-8} 
                          & DOME                         & \multicolumn{1}{c|}{31.83} & \multicolumn{1}{c|}{42.45}   & 20.48  & \multicolumn{1}{c|}{22.20} & \multicolumn{1}{c|}{36.67}   & 16.47  \\ \hline
\end{tabular}
}
\end{table}

==> tab/classification.tex <==

\begin{table*}[hbtp!]
\centering
\caption{{The performance of intent classification for code comments\lin{Del NB}}}
\label{table:classification}
\resizebox{\textwidth}{!}{

\begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{2}[0]{*}{Method} & \multicolumn{3}{c|}{What}                                    & \multicolumn{3}{c|}{Why}                                     & \multicolumn{3}{c|}{Usage}                                   & \multicolumn{3}{c|}{Done}                                    & \multicolumn{3}{c|}{Property}                                & \multicolumn{3}{c|}{Others}                                  & \multicolumn{3}{c|}{Macro-Average}                                   \\ \cline{2-22} 
                        & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   \\ \hline
LGBM                    & \multicolumn{1}{c|}{87.4} & \multicolumn{1}{c|}{92.3} & 89.8 & \multicolumn{1}{c|}{81.5} & \multicolumn{1}{c|}{76.8} & 79.0 & \multicolumn{1}{c|}{89.9} & \multicolumn{1}{c|}{72.5} & 80.1 & \multicolumn{1}{c|}{71.6} & \multicolumn{1}{c|}{65.8} & 68.5 & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{89.7} & 90.2 & \multicolumn{1}{c|}{12.6} & \multicolumn{1}{c|}{6.4}  & 8.4  & \multicolumn{1}{c|}{72.3} & \multicolumn{1}{c|}{67.2} & 69.3 \\ \hline
RF                      & \multicolumn{1}{c|}{83.9} & \multicolumn{1}{c|}{94.3} & 88.8 & \multicolumn{1}{c|}{84.0} & \multicolumn{1}{c|}{73.2} & 78.2 & \multicolumn{1}{c|}{92.3} & \multicolumn{1}{c|}{70.3} & 79.6 & \multicolumn{1}{c|}{75.8} & \multicolumn{1}{c|}{54.5} & 63.4 & \multicolumn{1}{c|}{90.9} & \multicolumn{1}{c|}{89.3} & 90.0 & \multicolumn{1}{c|}{39.9} & \multicolumn{1}{c|}{29.7} & 30.3 & \multicolumn{1}{c|}{77.8} & \multicolumn{1}{c|}{68.5} & 71.7 \\ \hline
NB                      & \multicolumn{1}{c|}{59.1} & \multicolumn{1}{c|}{99.8} & 74.2 & \multicolumn{1}{c|}{94.1} & \multicolumn{1}{c|}{8.7}  & 15.8 & \multicolumn{1}{c|}{70.0} & \multicolumn{1}{c|}{1.9}  & 3.6  & \multicolumn{1}{c|}{78.8} & \multicolumn{1}{c|}{3.3}  & 6.2  & \multicolumn{1}{c|}{95.2} & \multicolumn{1}{c|}{17.9} & 30.1 & \multicolumn{1}{c|}{0.0}  & \multicolumn{1}{c|}{0.0}  & 0.0  & \multicolumn{1}{c|}{66.2} & \multicolumn{1}{c|}{21.9} & 21.7 \\ \hline
DT                      & \multicolumn{1}{c|}{86.3} & \multicolumn{1}{c|}{87.0} & 86.6 & \multicolumn{1}{c|}{73.7} & \multicolumn{1}{c|}{74.0} & 73.8 & \multicolumn{1}{c|}{74.0} & \multicolumn{1}{c|}{69.5} & 71.5 & \multicolumn{1}{c|}{63.0} & \multicolumn{1}{c|}{59.9} & 61.3 & \multicolumn{1}{c|}{87.8} & \multicolumn{1}{c|}{86.8} & 87.2 & \multicolumn{1}{c|}{16.6} & \multicolumn{1}{c|}{32.5} & 20.6 & \multicolumn{1}{c|}{68.3} & \multicolumn{1}{c|}{66.9} & 66.8 \\ \hline
CNN                     & \multicolumn{1}{c|}{87.4} & \multicolumn{1}{c|}{93.3} & 90.2 & \multicolumn{1}{c|}{82.7} & \multicolumn{1}{c|}{77.3} & 79.9 & \multicolumn{1}{c|}{90.4} & \multicolumn{1}{c|}{71.3} & 79.5 & \multicolumn{1}{c|}{71.8} & \multicolumn{1}{c|}{65.7} & 68.6 & \multicolumn{1}{c|}{94.5} & \multicolumn{1}{c|}{89.4} & 91.8 & \multicolumn{1}{c|}{82.1} & \multicolumn{1}{c|}{29.2} & 41.5 & \multicolumn{1}{c|}{84.8} & \multicolumn{1}{c|}{71.0} & 75.3 \\ \hline
BiLSTM                  & \multicolumn{1}{c|}{88.4} & \multicolumn{1}{c|}{89.0} & 88.6 & \multicolumn{1}{c|}{78.5} & \multicolumn{1}{c|}{74.6} & 76.4 & \multicolumn{1}{c|}{81.0} & \multicolumn{1}{c|}{62.8} & 70.4 & \multicolumn{1}{c|}{60.5} & \multicolumn{1}{c|}{68.8} & 64.2 & \multicolumn{1}{c|}{96.1} & \multicolumn{1}{c|}{88.2} & 92.0 & \multicolumn{1}{c|}{10.0} & \multicolumn{1}{c|}{0.9}  & 1.7  & \multicolumn{1}{c|}{69.1} & \multicolumn{1}{c|}{64.1} & 65.5 \\ \hline
BiLSTM-Attn               & \multicolumn{1}{c|}{87.3} & \multicolumn{1}{c|}{91.5} & 89.3 & \multicolumn{1}{c|}{79.5} & \multicolumn{1}{c|}{75.2} & 77.2 & \multicolumn{1}{c|}{80.2} & \multicolumn{1}{c|}{68.1} & 73.3 & \multicolumn{1}{c|}{68.2} & \multicolumn{1}{c|}{67.3} & 67.7 & \multicolumn{1}{c|}{96.1} & \multicolumn{1}{c|}{88.6} & 92.1 & \multicolumn{1}{c|}{0.0}  & \multicolumn{1}{c|}{0.0}  & 0.0  & \multicolumn{1}{c|}{68.5} & \multicolumn{1}{c|}{65.1} & 66.6 \\ \hline
\rowcolor{gray!25}{\ltool}                    & \multicolumn{1}{c|}{\textbf{92.5}} & \multicolumn{1}{c|}{\textbf{93.5}} & \textbf{93.0} & \multicolumn{1}{c|}{\textbf{87.1}} & \multicolumn{1}{c|}{\textbf{86.1}} & \textbf{86.6 }& \multicolumn{1}{c|}{\textbf{93.0}} & \multicolumn{1}{c|}{\textbf{86.6}} & \textbf{89.6 }& \multicolumn{1}{c|}{\textbf{78.6}} & \multicolumn{1}{c|}{\textbf{79.2}} & \textbf{78.9 }& \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{\textbf{92.9}} & \textbf{94.6 }& \multicolumn{1}{c|}{\textbf{99.3}} & \multicolumn{1}{c|}{\textbf{90.7}} & \textbf{94.7 }& \multicolumn{1}{c|}{\textbf{91.1}} & \multicolumn{1}{c|}{\textbf{88.2}} & \textbf{89.6} \\ \hline
\end{tabular}
}
\end{table*}

==> tab/classification_v2.tex <==

\begin{table*}[hbtp!]
\centering
\caption{{The performance of intent classification for code comments}}
\label{table:classification}
\resizebox{\textwidth}{!}{

\begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{2}[0]{*}{Method} & \multicolumn{3}{c|}{What}                                    & \multicolumn{3}{c|}{Why}                                     & \multicolumn{3}{c|}{Usage}                                   & \multicolumn{3}{c|}{Done}                                    & \multicolumn{3}{c|}{Property}                                & \multicolumn{3}{c|}{Others}                                  & \multicolumn{3}{c|}{Macro-Average}                                   \\ \cline{2-22} 
                        & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   & \multicolumn{1}{c|}{P}    & \multicolumn{1}{c|}{R}    & F1   \\ \hline
LGBM                    & \multicolumn{1}{c|}{87.4} & \multicolumn{1}{c|}{92.3} & 89.8 & \multicolumn{1}{c|}{81.5} & \multicolumn{1}{c|}{76.8} & 79.0 & \multicolumn{1}{c|}{89.9} & \multicolumn{1}{c|}{72.5} & 80.1 & \multicolumn{1}{c|}{71.6} & \multicolumn{1}{c|}{65.8} & 68.5 & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{89.7} & 90.2 & \multicolumn{1}{c|}{12.6} & \multicolumn{1}{c|}{6.4}  & 8.4  & \multicolumn{1}{c|}{72.3} & \multicolumn{1}{c|}{67.2} & 69.3 \\ \hline
RF                      & \multicolumn{1}{c|}{83.9} & \multicolumn{1}{c|}{94.3} & 88.8 & \multicolumn{1}{c|}{84.0} & \multicolumn{1}{c|}{73.2} & 78.2 & \multicolumn{1}{c|}{92.3} & \multicolumn{1}{c|}{70.3} & 79.6 & \multicolumn{1}{c|}{75.8} & \multicolumn{1}{c|}{54.5} & 63.4 & \multicolumn{1}{c|}{90.9} & \multicolumn{1}{c|}{89.3} & 90.0 & \multicolumn{1}{c|}{39.9} & \multicolumn{1}{c|}{29.7} & 30.3 & \multicolumn{1}{c|}{77.8} & \multicolumn{1}{c|}{68.5} & 71.7 \\ \hline
DT                      & \multicolumn{1}{c|}{86.3} & \multicolumn{1}{c|}{87.0} & 86.6 & \multicolumn{1}{c|}{73.7} & \multicolumn{1}{c|}{74.0} & 73.8 & \multicolumn{1}{c|}{74.0} & \multicolumn{1}{c|}{69.5} & 71.5 & \multicolumn{1}{c|}{63.0} & \multicolumn{1}{c|}{59.9} & 61.3 & \multicolumn{1}{c|}{87.8} & \multicolumn{1}{c|}{86.8} & 87.2 & \multicolumn{1}{c|}{16.6} & \multicolumn{1}{c|}{32.5} & 20.6 & \multicolumn{1}{c|}{68.3} & \multicolumn{1}{c|}{66.9} & 66.8 \\ \hline
CNN                     & \multicolumn{1}{c|}{87.4} & \multicolumn{1}{c|}{93.3} & 90.2 & \multicolumn{1}{c|}{82.7} & \multicolumn{1}{c|}{77.3} & 79.9 & \multicolumn{1}{c|}{90.4} & \multicolumn{1}{c|}{71.3} & 79.5 & \multicolumn{1}{c|}{71.8} & \multicolumn{1}{c|}{65.7} & 68.6 & \multicolumn{1}{c|}{94.5} & \multicolumn{1}{c|}{89.4} & 91.8 & \multicolumn{1}{c|}{82.1} & \multicolumn{1}{c|}{29.2} & 41.5 & \multicolumn{1}{c|}{84.8} & \multicolumn{1}{c|}{71.0} & 75.3 \\ \hline
BiLSTM                  & \multicolumn{1}{c|}{88.4} & \multicolumn{1}{c|}{89.0} & 88.6 & \multicolumn{1}{c|}{78.5} & \multicolumn{1}{c|}{74.6} & 76.4 & \multicolumn{1}{c|}{81.0} & \multicolumn{1}{c|}{62.8} & 70.4 & \multicolumn{1}{c|}{60.5} & \multicolumn{1}{c|}{68.8} & 64.2 & \multicolumn{1}{c|}{96.1} & \multicolumn{1}{c|}{88.2} & 92.0 & \multicolumn{1}{c|}{10.0} & \multicolumn{1}{c|}{0.9}  & 1.7  & \multicolumn{1}{c|}{69.1} & \multicolumn{1}{c|}{64.1} & 65.5 \\ \hline
BiLSTM-Attn               & \multicolumn{1}{c|}{87.3} & \multicolumn{1}{c|}{91.5} & 89.3 & \multicolumn{1}{c|}{79.5} & \multicolumn{1}{c|}{75.2} & 77.2 & \multicolumn{1}{c|}{80.2} & \multicolumn{1}{c|}{68.1} & 73.3 & \multicolumn{1}{c|}{68.2} & \multicolumn{1}{c|}{67.3} & 67.7 & \multicolumn{1}{c|}{96.1} & \multicolumn{1}{c|}{88.6} & 92.1 & \multicolumn{1}{c|}{0.0}  & \multicolumn{1}{c|}{0.0}  & 0.0  & \multicolumn{1}{c|}{68.5} & \multicolumn{1}{c|}{65.1} & 66.6 \\ \hline
\rowcolor{gray!25}{\ltool}                    & \multicolumn{1}{c|}{\textbf{92.5}} & \multicolumn{1}{c|}{\textbf{93.5}} & \textbf{93.0} & \multicolumn{1}{c|}{\textbf{87.1}} & \multicolumn{1}{c|}{\textbf{86.1}} & \textbf{86.6 }& \multicolumn{1}{c|}{\textbf{93.0}} & \multicolumn{1}{c|}{\textbf{86.6}} & \textbf{89.6 }& \multicolumn{1}{c|}{\textbf{78.6}} & \multicolumn{1}{c|}{\textbf{79.2}} & \textbf{78.9 }& \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{\textbf{92.9}} & \textbf{94.6 }& \multicolumn{1}{c|}{\textbf{99.3}} & \multicolumn{1}{c|}{\textbf{90.7}} & \textbf{94.7 }& \multicolumn{1}{c|}{\textbf{91.1}} & \multicolumn{1}{c|}{\textbf{88.2}} & \textbf{89.6} \\ \hline
\end{tabular}
}
\end{table*}

==> tab/dataset.tex <==
\begin{table}[hbtp!]
\centering
\caption{Statistic of Funcom and TLC datasets}
\label{table:dataset}
\resizebox{0.7\columnwidth}{!}{

\begin{tabular}{|cc|c|c|c|}
\hline
\multicolumn{2}{|c|}{}                                      & Train     & Valid  & Test   \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{Funcom}}    & What     & 684,121   & 36,525 & 42,238 \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Why      & 152,320   & 8,317  & 8,275  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Usage    & 24,862    & 1,403  & 1,278  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Done     & 150,432   & 7,585  & 8,269  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Property & 167,188   & 8,553  & 9,199  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & All      & 1,178,923 & 62,383 & 69,259 \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{TLC}} & What     & 29,654    & 4,177  & 2,773  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Why      & 6,219     & 889    & 600    \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Usage    & 886       & 127    & 72     \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Done     & 11,698    & 1,605  & 1,089  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & Property & 5,071     & 757    & 451    \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                           & All      & 53,528    & 7,555  & 4,985  \\ \hline
\end{tabular}
}
\end{table}

==> tab/metrics.tex <==

\begin{table}[hbtp!]
\centering
\caption{{Performances of {\tool} and baselines on each intent category}}
\label{table:metircs}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|c|c|c|ccc|ccc|}
\hline
\multirow{2}{*}{}   & \multirow{2}{*}{Methods}   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Training\\ Data\end{tabular}} & \multicolumn{3}{c|}{Funcom}                                                                & \multicolumn{3}{c|}{TLC}                                                                   \\ \cline{4-9} 
                          &                            &                                                                          & \multicolumn{1}{c|}{BLEU}           & \multicolumn{1}{c|}{ROUGE-L}          & METEOR         & \multicolumn{1}{c|}{BLEU}           & \multicolumn{1}{c|}{ROUGE-L}          & METEOR         \\ \hline
\multirow{7}{*}{\rotatebox{90}{What}}     & \multirow{2}{*}{Rencos}    & All                                                                      & \multicolumn{1}{c|}{26.19}          & \multicolumn{1}{c|}{31.10}          & 14.61          & \multicolumn{1}{c|}{23.28}          & \multicolumn{1}{c|}{36.89}          & 16.02          \\ \cline{3-9} 
                          &                            & What                                                                     & \multicolumn{1}{c|}{28.83}          & \multicolumn{1}{c|}{32.44}          & 15.54          & \multicolumn{1}{c|}{23.20}          & \multicolumn{1}{c|}{36.08}          & 15.20          \\ \cline{2-9} 
                          & \multirow{2}{*}{EditSum}   & All                                                                      & \multicolumn{1}{c|}{27.58}          & \multicolumn{1}{c|}{31.06}          & 14.24          & \multicolumn{1}{c|}{21.34}          & \multicolumn{1}{c|}{33.73}          & 13.42          \\ \cline{3-9} 
                          &                            & What                                                                     & \multicolumn{1}{c|}{28.48}          & \multicolumn{1}{c|}{31.41}          & 14.48          & \multicolumn{1}{c|}{21.25}          & \multicolumn{1}{c|}{30.85}          & 13.15          \\ \cline{2-9} 
                          & \multirow{2}{*}{AST-Trans} & All                                                                      & \multicolumn{1}{c|}{27.84}          & \multicolumn{1}{c|}{38.28}          & 18.49          & \multicolumn{1}{c|}{23.42}          & \multicolumn{1}{c|}{34.24}          & 17.17          \\ \cline{3-9} 
                          &                            & What                                                                     & \multicolumn{1}{c|}{28.99}          & \multicolumn{1}{c|}{38.74}          & 18.80          & \multicolumn{1}{c|}{23.79}          & \multicolumn{1}{c|}{33.57}          & 16.38          \\ \cline{2-9} 
                          & DOME                       & All                                                                     & \multicolumn{1}{c|}{\textbf{33.29}} & \multicolumn{1}{c|}{\textbf{41.67}} & \textbf{20.53} & \multicolumn{1}{c|}{\textbf{25.39}} & \multicolumn{1}{c|}{\textbf{39.56}} & \textbf{18.22} \\ \hline
\multirow{7}{*}{\rotatebox{90}{Why}}      & \multirow{2}{*}{Rencos}    & All                                                                      & \multicolumn{1}{c|}{24.81}          & \multicolumn{1}{c|}{30.12}          & 14.21          & \multicolumn{1}{c|}{20.55}          & \multicolumn{1}{c|}{32.99}          & 14.54          \\ \cline{3-9} 
                          &                            & Why                                                                      & \multicolumn{1}{c|}{30.28}          & \multicolumn{1}{c|}{36.99}          & 17.09          & \multicolumn{1}{c|}{19.60}          & \multicolumn{1}{c|}{32.26}          & 11.98          \\ \cline{2-9} 
                          & \multirow{2}{*}{EditSum}   & All                                                                      & \multicolumn{1}{c|}{27.17}          & \multicolumn{1}{c|}{30.98}          & 14.66          & \multicolumn{1}{c|}{18.42}          & \multicolumn{1}{c|}{29.85}          & 11.81          \\ \cline{3-9} 
                          &                            & Why                                                                      & \multicolumn{1}{c|}{28.52}          & \multicolumn{1}{c|}{34.82}          & 15.20          & \multicolumn{1}{c|}{16.11}          & \multicolumn{1}{c|}{27.43}          & 9.21           \\ \cline{2-9} 
                          & \multirow{2}{*}{AST-Trans} & All                                                                      & \multicolumn{1}{c|}{25.96}          & \multicolumn{1}{c|}{35.74}          & 17.77          & \multicolumn{1}{c|}{19.31}          & \multicolumn{1}{c|}{29.37}          & 14.94          \\ \cline{3-9} 
                          &                            & Why                                                                      & \multicolumn{1}{c|}{29.41}          & \multicolumn{1}{c|}{39.67}          & 19.01          & \multicolumn{1}{c|}{19.23}          & \multicolumn{1}{c|}{27.25}          & 11.93          \\ \cline{2-9} 
                          & DOME                       & All                                                                      & \multicolumn{1}{c|}{\textbf{33.07}} & \multicolumn{1}{c|}{\textbf{42.31}} & \textbf{20.56} & \multicolumn{1}{c|}{\textbf{21.97}} & \multicolumn{1}{c|}{\textbf{35.31}} & \textbf{15.77} \\ \hline
\multirow{7}{*}{\rotatebox{90}{Usage}}    & \multirow{2}{*}{Rencos}    & All                                                                      & \multicolumn{1}{c|}{25.54}          & \multicolumn{1}{c|}{27.74}          & 13.34          & \multicolumn{1}{c|}{14.62}          & \multicolumn{1}{c|}{22.61}          & 10.21          \\ \cline{3-9} 
                          &                            & Usage                                                                    & \multicolumn{1}{c|}{30.77}          & \multicolumn{1}{c|}{37.70}          & 18.01          & \multicolumn{1}{c|}{12.47}          & \multicolumn{1}{c|}{21.67}          & 7.53           \\ \cline{2-9} 
                          & \multirow{2}{*}{EditSum}   & All                                                                      & \multicolumn{1}{c|}{25.25}          & \multicolumn{1}{c|}{27.25}          & 12.79          & \multicolumn{1}{c|}{14.00}          & \multicolumn{1}{c|}{21.51}          & 9.07           \\ \cline{3-9} 
                          &                            & Usage                                                                    & \multicolumn{1}{c|}{29.05}          & \multicolumn{1}{c|}{36.57}          & 16.94          & \multicolumn{1}{c|}{15.36}          & \multicolumn{1}{c|}{23.22}          & 11.01          \\ \cline{2-9} 
                          & \multirow{2}{*}{AST-Trans} & All                                                                      & \multicolumn{1}{c|}{24.93}          & \multicolumn{1}{c|}{30.90}          & 15.09          & \multicolumn{1}{c|}{13.24}          & \multicolumn{1}{c|}{18.20}          & 9.16           \\ \cline{3-9} 
                          &                            & Usage                                                                    & \multicolumn{1}{c|}{29.75}          & \multicolumn{1}{c|}{35.85}          & 17.08          & \multicolumn{1}{c|}{12.52}          & \multicolumn{1}{c|}{16.19}          & 7.49           \\ \cline{2-9} 
                          & DOME                       & All                                                                    & \multicolumn{1}{c|}{\textbf{31.63}} & \multicolumn{1}{c|}{\textbf{39.31}} & \textbf{19.34} & \multicolumn{1}{c|}{\textbf{17.16}} & \multicolumn{1}{c|}{\textbf{26.11}} & \textbf{12.36} \\ \hline
\multirow{7}{*}{\rotatebox{90}{Done}}     & \multirow{2}{*}{Rencos}    & All                                                                      & \multicolumn{1}{c|}{19.84}          & \multicolumn{1}{c|}{29.28}          & 12.53          & \multicolumn{1}{c|}{18.58}          & \multicolumn{1}{c|}{33.73}          & 13.12          \\ \cline{3-9} 
                          &                            & Done                                                                     & \multicolumn{1}{c|}{25.02}          & \multicolumn{1}{c|}{33.93}          & 14.64          & \multicolumn{1}{c|}{18.15}          & \multicolumn{1}{c|}{33.17}          & 12.76          \\ \cline{2-9} 
                          & \multirow{2}{*}{EditSum}   & All                                                                      & \multicolumn{1}{c|}{22.22}          & \multicolumn{1}{c|}{29.73}          & 12.62          & \multicolumn{1}{c|}{16.84}          & \multicolumn{1}{c|}{31.18}          & 11.12          \\ \cline{3-9} 
                          &                            & Done                                                                     & \multicolumn{1}{c|}{23.85}          & \multicolumn{1}{c|}{33.45}          & 13.43          & \multicolumn{1}{c|}{13.70}          & \multicolumn{1}{c|}{27.52}          & 8.51           \\ \cline{2-9} 
                          & \multirow{2}{*}{AST-Trans} & All                                                                      & \multicolumn{1}{c|}{19.65}          & \multicolumn{1}{c|}{33.60}          & 14.40          & \multicolumn{1}{c|}{17.61}          & \multicolumn{1}{c|}{30.32}          & 13.29          \\ \cline{3-9} 
                          &                            & Done                                                                     & \multicolumn{1}{c|}{22.91}          & \multicolumn{1}{c|}{36.03}          & 15.57          & \multicolumn{1}{c|}{17.76}          & \multicolumn{1}{c|}{29.85}          & 12.72          \\ \cline{2-9} 
                          & DOME                       & All                                                                     & \multicolumn{1}{c|}{\textbf{26.98}} & \multicolumn{1}{c|}{\textbf{39.52}} & \textbf{17.65} & \multicolumn{1}{c|}{\textbf{20.48}} & \multicolumn{1}{c|}{\textbf{36.66}} & \textbf{14.73} \\ \hline
\multirow{7}{*}{\rotatebox{90}{Prop.}} & \multirow{2}{*}{Rencos}    & All                                                                      & \multicolumn{1}{c|}{25.57}          & \multicolumn{1}{c|}{35.60}          & 16.39          & \multicolumn{1}{c|}{23.82}          & \multicolumn{1}{c|}{38.85}          & 17.76          \\ \cline{3-9} 
                          &                            & Property                                                                 & \multicolumn{1}{c|}{30.12}          & \multicolumn{1}{c|}{42.15}          & 20.36          & \multicolumn{1}{c|}{23.83}          & \multicolumn{1}{c|}{41.07}          & 17.85          \\ \cline{2-9} 
                          & \multirow{2}{*}{EditSum}   & All                                                                      & \multicolumn{1}{c|}{26.79}          & \multicolumn{1}{c|}{36.09}          & 16.60          & \multicolumn{1}{c|}{22.35}          & \multicolumn{1}{c|}{37.74}          & 16.33          \\ \cline{3-9} 
                          &                            & Property                                                                 & \multicolumn{1}{c|}{28.29}          & \multicolumn{1}{c|}{41.00}          & 18.84          & \multicolumn{1}{c|}{19.45}          & \multicolumn{1}{c|}{36.65}          & 15.01          \\ \cline{2-9} 
                          & \multirow{2}{*}{AST-Trans} & All                                                                      & \multicolumn{1}{c|}{28.29}          & \multicolumn{1}{c|}{43.54}          & 20.73          & \multicolumn{1}{c|}{23.54}          & \multicolumn{1}{c|}{36.56}          & 18.47          \\ \cline{3-9} 
                          &                            & Property                                                                 & \multicolumn{1}{c|}{30.14}          & \multicolumn{1}{c|}{46.83}          & 23.10          & \multicolumn{1}{c|}{23.88}          & \multicolumn{1}{c|}{37.08}          & 18.03          \\ \cline{2-9} 
                          & DOME                       & All                                                                 & \multicolumn{1}{c|}{\textbf{34.18}} & \multicolumn{1}{c|}{\textbf{49.43}} & \textbf{24.32} & \multicolumn{1}{c|}{\textbf{26.01}} & \multicolumn{1}{c|}{\textbf{45.73}} & \textbf{21.29} \\ \hline \hline
\multirow{7}{*}{\rotatebox{90}{\textit{Average\&Time}}}  & \multirow{2}{*}{Rencos}    & All (1.5h)                                                                      & \multicolumn{1}{c|}{24.39}          & \multicolumn{1}{c|}{30.77}          & 14.22          & \multicolumn{1}{c|}{20.17}          & \multicolumn{1}{c|}{33.01}          & 14.33          \\ \cline{3-9} 
                          &                            & Intent (5h)                                                                   & \multicolumn{1}{c|}{29.00}          & \multicolumn{1}{c|}{36.64}          & 17.13          & \multicolumn{1}{c|}{19.45}          & \multicolumn{1}{c|}{32.85}          & 13.06          \\ \cline{2-9} 
                          & \multirow{2}{*}{EditSum}   & All                                                                      & \multicolumn{1}{c|}{25.80}          & \multicolumn{1}{c|}{31.02}          & 14.18          & \multicolumn{1}{c|}{18.59}          & \multicolumn{1}{c|}{30.80}          & 12.35          \\ \cline{3-9} 
                          &                            & Intent                                                                   & \multicolumn{1}{c|}{27.64}          & \multicolumn{1}{c|}{35.45}          & 15.78          & \multicolumn{1}{c|}{17.17}          & \multicolumn{1}{c|}{29.13}          & 11.38          \\ \cline{2-9} 
                          & \multirow{2}{*}{AST-Trans} & All                                                                      & \multicolumn{1}{c|}{25.33}          & \multicolumn{1}{c|}{36.41}          & 17.30          & \multicolumn{1}{c|}{19.42}          & \multicolumn{1}{c|}{29.74}          & 14.61          \\ \cline{3-9} 
                          &                            & Intent                                                                   & \multicolumn{1}{c|}{28.24}          & \multicolumn{1}{c|}{39.42}          & 18.71          & \multicolumn{1}{c|}{19.44}          & \multicolumn{1}{c|}{28.79}          & 13.31          \\ \cline{2-9} 
                          & DOME                       & All                                                                   & \multicolumn{1}{c|}{\textbf{31.83}} & \multicolumn{1}{c|}{\textbf{42.45}} & \textbf{20.48} & \multicolumn{1}{c|}{\textbf{22.20}} & \multicolumn{1}{c|}{\textbf{36.67}} & \textbf{16.47} \\ \hline
\end{tabular}
}
\end{table}
